Exploring Design and Governance Challenges in the Development of Privacy-Preserving Computation

Homomorphic encryption, secure multi-party computation, and differential privacy are part of an emerging class of Privacy Enhancing Technologies which share a common promise: to preserve privacy whilst also obtaining the benefits of computational analysis. Due to their relative novelty, complexity, and opacity, these technologies provoke a variety of novel questions for design and governance. We interviewed researchers, developers, industry leaders, policymakers, and designers involved in their deployment to explore motivations, expectations, perceived opportunities and barriers to adoption. This provided insight into several pertinent challenges facing the adoption of these technologies, including: how they might make a nebulous concept like privacy computationally tractable; how to make them more usable by developers; and how they could be explained and made accountable to stakeholders and wider society. We conclude with implications for the development, deployment, and responsible governance of these privacy-preserving computation techniques.

==> App_Protocol_Experts.tex <==



\section{Protocol For People in Research / Industry / Development }
*For these interviews we limited our scope to the privacy preserving computation PETs.

\begin{enumerate}
	\item \textbf{Background: }Tell us a bit about your experience with PETs \par

\begin{enumerate}
	\item What experience do you possess?\par

	\item How many years have you spent researching / engaging in this domain?\par

	\item What type of technologies (PETs) have you focused on?\par

	\item What sector best defines your role (Industry / Academia / policymaker etc)\par

\begin{enumerate}
	\item Govt. or private sector?\par


\end{enumerate}


\vspace{\baselineskip}

\end{enumerate}
	\item \textbf{Opportunities}\par

\begin{enumerate}
	\item \textbf{ }What do you think are the most promising (real world) applications of PETs?\par

\begin{enumerate}
	\item Which of these do you think are already pragmatic or realizable in the \textit{short term },\ i.e.,\ with the current state of these technologies?   (Short term $ \sim $ 1 year)\par

	\item What do you think are the most promising \textit{long term}\ applications?  (Long Term $ \sim $  5+ years)\par



\end{enumerate}
	\item If there were to be an incredible breakthrough, what would you want/expect/wish PETs to achieve?\par

	\item What do you think is the current state of PETs for real world usage\par

\begin{enumerate}
	\item Are there libraries for PETs?\par

\begin{enumerate}
	\item What\ do you  think about the state of those libraries ?\par

	\item Are they sufficient for broader adoption\par
	\item If not, what could industry/experts do about it?\par

\end{enumerate}
\end{enumerate}
	\item As\ an applied researcher what do you think about the state of theoretical research in your domain (ongoing  improvement?)?\par

	\item On a scale of 1-10, how much potential have the PETs already realized?\par
\vspace{\baselineskip}

\end{enumerate}
	\item \textbf{Barriers to adoption}
\begin{enumerate}
    \item  What do you think are the major barriers to more widespread adoption or wider use of PETs in the real world? \par
	\item What are the major blockers for adoption?\par

\begin{enumerate}
	\item What does the privacy vs time/cost/resources the trade-off for using PETs look like in your opinion?\par


\end{enumerate}
	\item How would you compare/define/separate (draw the boundaries) between different PETs (you’re aware of)?\par

	\item What common misunderstanding have you encountered about different PETs?\par

\begin{enumerate}
	\item What PETs do you think are the hardest to explain and why?\par


\end{enumerate}
	\item How do you think applied PETs are different from technologies like Machine Learning w.r.t. to ease of use?\par

\begin{enumerate}
	\item What are the major usability barriers?\par

\begin{enumerate}
	\item Which of these do you think can be addressed over time?\par


\end{enumerate}
\end{enumerate}
	\item \textit{(Only for Library Developers)} : What problem does your library solve?\par

\begin{enumerate}
	\item What kind of challenges do your users face?\par

\begin{enumerate}
	\item Which of these challenges are addressable and which of these are not?\par

	\item How do you plan to address the challenges you just discussed?\par


\end{enumerate}
\vspace{\baselineskip}

\end{enumerate}
\end{enumerate}
	\item \textbf{Explanations} : \par

\begin{enumerate}
	\item How would you explain a PET to a layman?\par

\begin{enumerate}
	\item What are the barriers have you faced in explaining a PET?\par


\end{enumerate}
	\item Have you personally had to explain PETs to a non-expert? In what contexts or capacity have you had to do so? \par

	\item Revisit a specific time where you tried to explain PETs to a non-expert. What were the challenges? What worked, what didn’t work?\par



\vspace{\baselineskip}

\end{enumerate}

	\item \textbf{Expectations}\par

\begin{enumerate}
	\item What problems / privacy concerns do you think PETs solve for:\par

\begin{enumerate}
	\item End-users\par

	\item Businesses\par


\end{enumerate}
	\item What do you think your role might be, if any, in defining and identifying problems PETs might solve?\par

	\item What do you think different stakeholders ( Businesses, end-users, developers, etc) must know about a PET to make informed choices?
\end{enumerate}
\end{enumerate}\par


==> App_Protocol_policy_design.tex <==
\section{Protocol For People in Policy / Design }

*For these interviews we limited our scope to the privacy preserving computation PETs.

\begin{enumerate}
	\item \textbf{Background: }Tell us a bit about your experience with PETs \par

\begin{enumerate}
	\item What experience do you possess?\par

	\item How many years have you spent researching / engaging in this domain?\par

	\item What type of technologies (PETs) have you focused on?\par

	\item What sector best defines your role (Industry / Academia / policymaker etc)\par

\begin{enumerate}
	\item Govt. or private sector?\par


\end{enumerate}


\vspace{\baselineskip}

\end{enumerate}
	\item \textbf{Opportunities }\par

\begin{enumerate}
	\item What do you think are the most promising (real world) applications of PETs? \par

\begin{enumerate}
	\item Are these realizable at the moment? \par

	\item Do these applications solve policy or regulatory problems, if so, what?\par

\begin{enumerate}
	\item If not, why not? What do they get wrong? How could they be modified to be more useful?\par


\end{enumerate}
\end{enumerate}
	\item If there were to be an incredible breakthrough, what would you want/expect/wish PETs to achieve? 
	(Any kind--- Technology/ Policy/ Regulatory etc)\par


	\item Do you think PETs solve real problems? Which problems and whose problems? \par

	\item Is there a demand for these technologies already? Or do we still need to motivate the use-case?\par

	\item What major (privacy) problems do you think still remain unsolved even with the use of these technologies?\\
\par


\end{enumerate}
	\item \textbf{Barriers to adoption}\par

\begin{enumerate}
	\item What do you think are the major barriers to more widespread adoption or wider use of PETs in the real world? \par

	\item Regulatory\ policy barriers :  Have regulators particularly encouraged adoption of these technologies? If so, how? If not, why not?\par

	\item Do you think current regulations like GDPR / HIPAA already encompass guidelines for such technologies?\par

	\item What roles, do you think, your peers could play in mitigating barriers to adoption of PETs ?\par

	\item What role do you think other stakeholders (experts / developers) could play?\par


\vspace{\baselineskip}

\end{enumerate}
	\item \textbf{Explanations and Understanding}\par

\begin{enumerate}
	\item What kind of technical understanding, of these technologies, someone in your position would need?\par

\begin{enumerate}
	\item To what level of granularity?\par

	\item How did you get there (getting that understanding)?\par


\end{enumerate}
	\item \textbf{Explaining to non-experts (context): }Have you personally had to explain PETs to a non-expert? In what contexts or capacity have you had to do so? \par

	\item \textbf{Explaining to a non-expert (strategy): }Revisit a specific time where you tried to explain PETs to a non-expert. What were the challenges? What worked, what didn’t work? \\
\par


\end{enumerate}
	\item \textbf{Expectations}\par

\begin{enumerate}
	\item What problems / privacy concerns do you think PETs solve for :\par

\begin{enumerate}
	\item End-users\par

	\item Businesses\par

	\item What do you think your role might be, if any, in defining and identifying problems PETs might solve?\par


\end{enumerate}
	\item What do you think different stakeholders ( Businesses, end- users, developers, etc) should know about PETs to make informed choices?
\end{enumerate}
\end{enumerate}\par

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> recommendations.tex <==
\section{Recommendations}
\nitin{Not sure whether we need a separate section for this or we cover it in the discussion itself}
\reuben{i vote no}
